Towards Scalable SOAP Note Generation: A Weakly Supervised Multimodal Framework

Skin carcinoma is the most prevalent form of cancer globally, accounting for over $8 billion in annual healthcare expenditures. In clinical settings, physicians document patient visits using detailed SOAP (Subjective, Objective, Assessment, and Plan) notes. However, manually generating these notes is labor-intensive and contributes to clinician burnout. In this work, we propose a weakly supervised multimodal framework to generate clinically structured SOAP notes from limited inputs, including lesion images and sparse clinical text. Our approach reduces reliance on manual annotations, enabling scalable, clinically grounded documentation while alleviating clinician burden and reducing the need for large annotated data. Our method achieves performance comparable to GPT-4o, Claude, and DeepSeek Janus Pro across key clinical relevance metrics. To evaluate clinical quality, we introduce two novel metrics MedConceptEval and Clinical Coherence Score (CCS) which assess semantic alignment with expert medical concepts and input features, respectively.

==> 2_related.tex <==

\section{Related Works}
\label{sec:related}

Artificial intelligence has been widely applied in the medical domain for tasks such as medical image captioning \cite{cheng2025caparena}, clinical text summarization \cite{van2023clinical}, discharge note generation \cite{jung2024enhancing}, and medical question answering \cite{yan2024large}. Recent efforts have focused on generating clinical notes, especially SOAP notes, from Electronic Health Records (EHRs) and doctor-patient conversations. In \cite{li2024improving}, large language models (LLMs) are fine-tuned to generate K-SOAP notes, while \cite{chen2024exploring} evaluated generative models across general and SOAP-specific formats. Similar work has explored domains like pediatric rehabilitation \cite{amenyo2025assessment} and fine-tuning LLMs for efficient SOAP note generation \cite{leong2024efficient}. 

Earlier approaches to SOAP note generation, such as \cite{schloss2020towards,singh2023large}, used sequence-to-sequence models and transformer architectures trained on large dialogue datasets. Although general-purpose LLMs have improved clinical NLP tasks \cite{singhal2023large,yang2023large}, they often lack domain-specific reasoning and structured multimodal output capabilities.  While methods like \cite{ramprasad2023generating} have attempted to improve faithfulness in text-based settings, these methods heavily rely on large annotated dialogue corpora, which are difficult to obtain due to privacy concerns \cite{chen2024exploring}, and they remain text-centric without leveraging multimodal information, which is critical to fields like dermatology. SkinGPT-4 \cite{zhou2024pre} recently demonstrated that integrating clinical images and text using a multimodal LLM improves dermatological diagnostic reasoning. However, it is primarily designed for diagnostic prediction and lacks structured documentation capabilities. Specifically, it does not generate clinically formatted SOAP notes or support section-level reasoning required for clinical documentation. In contrast, our work focuses on end-to-end generation of structured SOAP notes from limited multimodal inputs, introducing weak supervision and domain-guided retrieval to ensure both clinical reliability and scalability.


% SkinGPT-4 \cite{zhou2024pre} recently demonstrated that integrating clinical images and text using a multimodal LLM improves dermatological diagnostic reasoning, but it does not produce structured documentation such as SOAP notes. Therefore, we propose a multimodal framework that takes only an input lesion image and related caption to generate structured SOAP notes, reducing reliance on large datasets including doctor-patient conversations and enhancing clinical reliability through domain-guided knowledge retrieval, particularly for skin lesion datasets.











==> 5_limit.tex <==
\section{Limitations and Future Work}
\label{sec:limit}

% While our weakly supervised multimodal framework shows strong promise for structured SOAP notes generation, it has few limitations. The quality of the generated SOAP notes remains dependent on the accuracy of the retrieved domain-specific knowledge, which may introduce biases or propagate incomplete information. Additionally, we utilized only a single dataset, as variations in metadata across different sources posed challenges for standardization, thereby limiting the model’s generalizability to broader clinical settings. Our evaluation was further constrained by a small set of expert-annotated samples, restricting large-scale validation. In Future work, we will focus on expanding to more diverse datasets, and incorporating human-in-the-loop refinement strategies. Furthermore, developing better evaluation benchmarks that track patient reasoning over time and support clinical decision-making could make automated clinical note generation much more useful in real-world healthcare settings.

While our weakly supervised multimodal framework shows strong promise for structured SOAP notes generation, it has few limitations. The quality of the generated SOAP notes remains dependent on the accuracy of the retrieved domain-specific knowledge, which may introduce biases or propagate incomplete information. Additionally, we utilized only a single dataset, as variations in metadata across different sources posed challenges for standardization. Our evaluation was further constrained by a small set of expert-annotated samples, restricting large-scale validation. Like most generative models, our approach may hallucinate when faced with ambiguous or unfamiliar inputs. Although retrieval-augmented generation helps reduce this risk by grounding outputs in clinical knowledge, additional safeguards are needed for real-world deployment. In Future work, we will focus on expanding to more diverse datasets, and incorporating human-in-the-loop refinement strategies. Furthermore, developing evaluation benchmarks that capture the progression of clinical reasoning across multiple encounters and support decision-making could significantly improve the utility of automated SOAP note generation in real-world healthcare settings.
